Angular Momentum Changes Due to Direct Impact Accretion in a Simplified Binary System

We model a circular mass-transferring binary system to calculate the exchange of angular momentum between stellar spins and the orbit due to direct impact of the mass transfer stream onto the surface of the accretor. We simulate mass transfer by calculating the ballistic motion of a point mass ejected from the $L_1$ point of the donor star, conserving the total linear and angular momentum of the system, and treating the stars as uniform density spheres with main sequence radii determined by their masses. We show that, contrary to previous assumptions in the literature, direct impact does not always act as a sink of orbital angular momentum and may in fact increase it by facilitating the transfer of angular momentum from the spin of the donor to the orbit. Here, we show an example of the exchange of angular momentum, as well as a measure of the orbital angular momentum changes for a variety of binary star systems with main sequence components.

==> abbrvs.tex <==
%% Personally Added Journal Definitions -- Jeremy Sepinsky 7-18-2010
\let\jnl@style=\rmfamily
\def\ref@jnl#1{{\jnl@style#1}}%
\newcommand\aj{\ref@jnl{AJ}}%
          % Astronomical Journal
\newcommand\actaa{\ref@jnl{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{\ref@jnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\ref@jnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\ref@jnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\ref@jnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\ref@jnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\ref@jnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\ref@jnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\ref@jnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\ref@jnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\ref@jnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\ref@jnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{\ref@jnl{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\ref@jnl{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\ref@jnl{Icarus}}%
  % Icarus
\newcommand\jcap{\ref@jnl{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\ref@jnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\ref@jnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\ref@jnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{\ref@jnl{New A}}%
  % New Astronomy
\newcommand\nar{\ref@jnl{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{\ref@jnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\ref@jnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\ref@jnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\ref@jnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\ref@jnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\ref@jnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{\ref@jnl{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\ref@jnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\ref@jnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\ref@jnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\ref@jnl{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\ref@jnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\ref@jnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\ref@jnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\ref@jnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\ref@jnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\ref@jnl{Nature}}%
          % Nature
\newcommand\iaucirc{\ref@jnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\ref@jnl{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\ref@jnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\ref@jnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\ref@jnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\ref@jnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\ref@jnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\ref@jnl{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\ref@jnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\ref@jnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\ref@jnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\ref@jnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\ref@jnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\ref@jnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\ref@jnl{Proc.~SPIE}}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
\newcommand\phn{\phantom{0}}%
\newcommand\phd{\phantom{.}}%










\endinput
%%
%% End of file `aipproc.cls'.

